Floorplan: Spatial Layout in Memory Management Systems

In modern runtime systems, memory layout calculations are hand-coded in systems languages. Primitives in these languages are not powerful enough to describe a rich set of layouts, leading to reliance on ad-hoc macros, numerous interrelated static constants, and other boilerplate code. Memory management policies must also carefully orchestrate their application of address calculations in order to modify memory cooperatively, a task ill-suited to low-level systems languages at hand which lack proper safety mechanisms. In this paper we introduce Floorplan, a declarative language for specifying high level memory layouts. Constraints formerly implemented by describing how to compute locations are, in Floorplan, defined declaratively using explicit layout constructs. The challenge here was to discover constructs capable of sufficiently enabling the automatic generation of address calculations. Floorplan is implemented as a compiler for generating a Rust library. In a case study of an existing implementation of the immix garbage collection algorithm, Floorplan eliminates 55 out of the 63 unsafe lines of code: 100\% of unsafe lines pertaining to memory safety.

==> fsm/1.tex <==

\begin{center}
\begin{tikzpicture}[scale=0.1]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (16.3,-20.3) circle (3);
\draw (16.3,-20.3) node {hd};
\draw [black] (34.2,-20.3) circle (3);
\draw (34.2,-20.3) node {tl};
\draw [black] (34.2,-9.3) circle (3);
\draw (34.2,-9.3) node {$\texttt{K}_0$};
\draw [black] (16.3,-31.5) circle (3);
\draw (16.3,-31.5) node {$1$};
\draw [black] (16.3,-31.5) circle (2.4);
\draw [black] (25.9,-31.5) circle (3);
\draw (25.9,-31.5) node {lft};
\draw [black] (34.2,-31.5) circle (3);
\draw (34.2,-31.5) node {rgt};
\draw [black] (25.9,-46) circle (3);
\draw (25.9,-46) node {$1$};
\draw [black] (25.9,-46) circle (2.4);
\draw [black] (34.2,-46) circle (3);
\draw (34.2,-46) node {$1$};
\draw [black] (34.2,-46) circle (2.4);
\draw [black] (42.8,-46) circle (3);
\draw (42.8,-46) node {$1$};
\draw [black] (42.8,-46) circle (2.4);
\draw [black] (51.6,-45.9) circle (3);
\draw (51.6,-45.9) node {$1$};
\draw [black] (51.6,-45.9) circle (2.4);
\draw [black] (31.64,-10.87) -- (18.86,-18.73);
\fill [black] (18.86,-18.73) -- (19.8,-18.74) -- (19.28,-17.88);
\draw [black] (34.2,-12.3) -- (34.2,-17.3);
\fill [black] (34.2,-17.3) -- (34.7,-16.5) -- (33.7,-16.5);
\draw [black] (16.3,-23.3) -- (16.3,-28.5);
\fill [black] (16.3,-28.5) -- (16.8,-27.7) -- (15.8,-27.7);
\draw [black] (32.41,-22.71) -- (27.69,-29.09);
\fill [black] (27.69,-29.09) -- (28.56,-28.74) -- (27.76,-28.15);
\draw [black] (34.2,-23.3) -- (34.2,-28.5);
\fill [black] (34.2,-28.5) -- (34.7,-27.7) -- (33.7,-27.7);
\draw [black] (25.9,-34.5) -- (25.9,-43);
\fill [black] (25.9,-43) -- (26.4,-42.2) -- (25.4,-42.2);
\draw [black] (34.2,-34.5) -- (34.2,-43);
\fill [black] (34.2,-43) -- (34.7,-42.2) -- (33.7,-42.2);
\draw [black] (35.73,-34.08) -- (41.27,-43.42);
\fill [black] (41.27,-43.42) -- (41.29,-42.48) -- (40.43,-42.99);
\draw [black] (36.51,-33.41) -- (49.29,-43.99);
\fill [black] (49.29,-43.99) -- (48.99,-43.09) -- (48.35,-43.86);
\end{tikzpicture}
\end{center}



==> fsm/2.tex <==

\begin{center}
\begin{tikzpicture}[scale=0.1]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (16.3,-20.3) circle (3);
\draw (16.3,-20.3) node {hd};
\draw [black] (34.2,-20.3) circle (3);
\draw (34.2,-20.3) node {tl};
\draw [black] (34.2,-9.3) circle (3);
\draw (34.2,-9.3) node {$\texttt{K}_1$};
\draw [black] (16.3,-31.5) circle (3);
\draw (16.3,-31.5) node {$1$};
\draw [black] (16.3,-31.5) circle (2.4);
\draw [black] (25.9,-31.5) circle (3);
\draw (25.9,-31.5) node {lft};
\draw [black] (34.2,-31.5) circle (3);
\draw (34.2,-31.5) node {rgt};
\draw [black] (25.9,-46) circle (3);
\draw (25.9,-46) node {$1$};
\draw [black] (25.9,-46) circle (2.4);
\draw [black] (43,-46) circle (3);
\draw (43,-46) node {$1$};
\draw [black] (43,-46) circle (2.4);
\draw [black] (43,-31.5) circle (3);
\draw (43,-31.5) node {lft};
\draw [black] (51.7,-31.5) circle (3);
\draw (51.7,-31.5) node {rgt};
\draw [black] (9.7,-31.5) circle (3);
\draw (9.7,-31.5) node {$1$};
\draw [black] (9.7,-31.5) circle (2.4);
\draw [black] (51.7,-46) circle (3);
\draw (51.7,-46) node {$1$};
\draw [black] (51.7,-46) circle (2.4);
\draw [black] (31.64,-10.87) -- (18.86,-18.73);
\fill [black] (18.86,-18.73) -- (19.8,-18.74) -- (19.28,-17.88);
\draw [black] (34.2,-12.3) -- (34.2,-17.3);
\fill [black] (34.2,-17.3) -- (34.7,-16.5) -- (33.7,-16.5);
\draw [black] (16.3,-23.3) -- (16.3,-28.5);
\fill [black] (16.3,-28.5) -- (16.8,-27.7) -- (15.8,-27.7);
\draw [black] (32.41,-22.71) -- (27.69,-29.09);
\fill [black] (27.69,-29.09) -- (28.56,-28.74) -- (27.76,-28.15);
\draw [black] (34.2,-23.3) -- (34.2,-28.5);
\fill [black] (34.2,-28.5) -- (34.7,-27.7) -- (33.7,-27.7);
\draw [black] (25.9,-34.5) -- (25.9,-43);
\fill [black] (25.9,-43) -- (26.4,-42.2) -- (25.4,-42.2);
\draw [black] (36.05,-22.66) -- (41.15,-29.14);
\fill [black] (41.15,-29.14) -- (41.05,-28.2) -- (40.26,-28.82);
\draw [black] (36.73,-21.92) -- (49.17,-29.88);
\fill [black] (49.17,-29.88) -- (48.77,-29.03) -- (48.23,-29.87);
\draw [black] (43,-34.5) -- (43,-43);
\fill [black] (43,-43) -- (43.5,-42.2) -- (42.5,-42.2);
\draw [black] (14.78,-22.88) -- (11.22,-28.92);
\fill [black] (11.22,-28.92) -- (12.06,-28.48) -- (11.2,-27.97);
\draw [black] (51.7,-34.5) -- (51.7,-43);
\fill [black] (51.7,-43) -- (52.2,-42.2) -- (51.2,-42.2);
\end{tikzpicture}
\end{center}



==> fsm/3.tex <==

\begin{center}
\begin{tikzpicture}[scale=0.1]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (16.3,-20.3) circle (3);
\draw (16.3,-20.3) node {hd};
\draw [black] (34.2,-20.3) circle (3);
\draw (34.2,-20.3) node {tl};
\draw [black] (34.2,-9.3) circle (3);
\draw (34.2,-9.3) node {$\texttt{K}_2$};
\draw [black] (16.3,-31.5) circle (3);
\draw (16.3,-31.5) node {$1$};
\draw [black] (16.3,-31.5) circle (2.4);
\draw [black] (25.9,-31.5) circle (3);
\draw (25.9,-31.5) node {lft};
\draw [black] (34.2,-31.5) circle (3);
\draw (34.2,-31.5) node {rgt};
\draw [black] (25.9,-46) circle (3);
\draw (25.9,-46) node {$1$};
\draw [black] (25.9,-46) circle (2.4);
\draw [black] (43,-46) circle (3);
\draw (43,-46) node {$1$};
\draw [black] (43,-46) circle (2.4);
\draw [black] (43,-31.5) circle (3);
\draw (43,-31.5) node {lft};
\draw [black] (51.7,-31.5) circle (3);
\draw (51.7,-31.5) node {rgt};
\draw [black] (9.7,-31.5) circle (3);
\draw (9.7,-31.5) node {$1$};
\draw [black] (9.7,-31.5) circle (2.4);
\draw [black] (34.2,-46) circle (3);
\draw (34.2,-46) node {$1$};
\draw [black] (34.2,-46) circle (2.4);
\draw [black] (31.64,-10.87) -- (18.86,-18.73);
\fill [black] (18.86,-18.73) -- (19.8,-18.74) -- (19.28,-17.88);
\draw [black] (34.2,-12.3) -- (34.2,-17.3);
\fill [black] (34.2,-17.3) -- (34.7,-16.5) -- (33.7,-16.5);
\draw [black] (16.3,-23.3) -- (16.3,-28.5);
\fill [black] (16.3,-28.5) -- (16.8,-27.7) -- (15.8,-27.7);
\draw [black] (32.41,-22.71) -- (27.69,-29.09);
\fill [black] (27.69,-29.09) -- (28.56,-28.74) -- (27.76,-28.15);
\draw [black] (34.2,-23.3) -- (34.2,-28.5);
\fill [black] (34.2,-28.5) -- (34.7,-27.7) -- (33.7,-27.7);
\draw [black] (25.9,-34.5) -- (25.9,-43);
\fill [black] (25.9,-43) -- (26.4,-42.2) -- (25.4,-42.2);
\draw [black] (36.05,-22.66) -- (41.15,-29.14);
\fill [black] (41.15,-29.14) -- (41.05,-28.2) -- (40.26,-28.82);
\draw [black] (36.73,-21.92) -- (49.17,-29.88);
\fill [black] (49.17,-29.88) -- (48.77,-29.03) -- (48.23,-29.87);
\draw [black] (43,-34.5) -- (43,-43);
\fill [black] (43,-43) -- (43.5,-42.2) -- (42.5,-42.2);
\draw [black] (14.78,-22.88) -- (11.22,-28.92);
\fill [black] (11.22,-28.92) -- (12.06,-28.48) -- (11.2,-27.97);
\draw [black] (34.2,-34.5) -- (34.2,-43);
\fill [black] (34.2,-43) -- (34.7,-42.2) -- (33.7,-42.2);
\end{tikzpicture}
\end{center}


